Batch Active Learning at Scale

The ability to train complex and highly effective models often requires an abundance of training data, which can easily become a bottleneck in cost, time, and computational resources. Batch active learning, which adaptively issues batched queries to a labeling oracle, is a common approach for addressing this problem. The practical benefits of batch sampling come with the downside of less adaptivity and the risk of sampling redundant examples within a batch -- a risk that grows with the batch size. In this work, we analyze an efficient active learning algorithm, which focuses on the large batch setting. In particular, we show that our sampling method, which combines notions of uncertainty and diversity, easily scales to batch sizes (100K-1M) several orders of magnitude larger than used in previous studies and provides significant improvements in model training efficiency compared to recent baselines. Finally, we provide an initial theoretical analysis, proving label complexity guarantees for a related sampling method, which we show is approximately equivalent to our sampling method in specific settings.

==> sampling_analysis.tex <==
%
\section{Sampling analysis}

%
\textbf{Setup}.
Consider a supervised learning problem over a training sample $S = \{ ( x_n, y_n ) \}_{n = 1}^N$,
with hypothesis class $\mathscr{H}$ and loss function $\ell$.
Let $h^*$ denote the empirical risk minimiser,
i.e.,
\begin{align*}
    h^* &\defEq \underset{h \in \mathscr{H}}{\operatorname{argmin}} \, R( h; S ) \\
    R( h; S ) &\defEq \frac{1}{N} \sum_{n \in [N]} \ell( y_n, h( x_n ) ).
\end{align*}
Our interest is in settings where $N$ is prohibitively large, so that computing $h^*$ is expensive.
We would thus like to find some $S' \subset S$
with $N' \defEq | S' | \ll N$,
so that the empirical risk minimiser on $S'$ attains similar loss as $h^*$;
that is, if
\begin{align*}
    h' &\defEq \underset{h \in \mathscr{H}}{\operatorname{argmin}} \, R( h; S' ) \\
    R( h; S' ) &\defEq \frac{1}{N'} \sum_{n' \in [N']} \ell( y_{n'}, h( x_{n'} ) ),
\end{align*}
then
we would like $R( h'; S ) \leq R( h^*; S ) + \epsilon$ for suitable $\epsilon > 0$.

In constructing $S'$, we have a \emph{constraint}:
we are not allowed to inspect the entire sample $S$.
This poses a considerable challenge,
but we are given access to a set of \emph{clusters} $\mathscr{C} = \{ C_1, \ldots, C_K \}$, where 
the $C_i's$ form a partition of the training instances $X = \{ x_n \}_{n = 1}^N$.
These clusters are assumed to be suitably tight and well-separated.
In an abuse of notation, denote by $C( x ) \in [ K ]$ the cluster corresponding to instance $x$.

%
\textbf{\color{Maroon}Remark}.
In settings where SGD does not need a full epoch to converge,
a random subsample of the $S$ can suffice for constructing $S'$.
Note that SGD may find a solution that generalises well even if it does not minimise the empirical risk exactly~\citep{Bottou:2007}.

%
\textbf{\color{Maroon}Remark}.
There is potentially a mismatch between the setup above, and the active learning setting that is the primary focus of the experiments.
In particular, in the active learning setting one must query each example to obtain a label.
The above problem is one of subset selection.

%
\textbf{\color{Maroon}Remark}.
The goal stated above concerns approximating the empirical risk over $S$.
One may also be interested in controlling the population risk $R( h'; \mathbb{P} )$ (where $S \sim \mathbb{P}^N$), which can follow from standard uniform convergence bounds.

\

%
\textbf{Current algorithm}.
The gist of the current algorithm is the following iterative procedure:
\begin{enumerate}
    \item draw a large pool of samples $T \subset S$ uniformly at random
    \item under current hypothesis $h$, compute the \emph{margin} of each sample in $T$, i.e.,
    $$ \gamma( x, y ) \defEq h_{y}( x ) - \max_{y' \neq y} h_{y'}( x ), $$
    where $h_y( x ) \in \mathbb{R}$ is the score assigned to label $y$ for instance $x$
    \item retain the top-$k$ lowest margin samples $T'$
    \item update the hypothesis using a round-robin schedule based on the clusters $C( x )$ for each $(x, y) \in T'$
    \item repeat step (1) until convergence
\end{enumerate}
In step (4) above, the round-robin schedule reduces potential redundancy in the model updates.
In particular, suppose there are samples $( x, y )$ and $( x', y )$ where $C( x ) = C( x' )$, and the clusters are suitably tight.
Under suitable Lipschitz assumptions on the loss and hypothesis class, we would expect the model gradients evaluated on these samples to be similar.
Intuitively,
then,
there is little value in using both samples to update the model.

A potential variant of step (4) would be to perform sampling based on the clusters, as opposed to a round-robin schedule.
Note that we may write the empirical risk as
\begin{align*}
    R( h; S ) &= \frac{1}{N} \sum_{k \in [K]} \sum_{( x, y ) \in C_k} \ell( y, h( x ) ) \\
    &= \sum_{k \in [K]} \frac{| C_k |}{N} \cdot \mathbb{E}_{( x, y ) \sim C_k}[  \ell( y, h( x ) ) ],
\end{align*}
which has an intuitive interpretation:
we average the loss over a cluster randomly drawn with probability proportional to the cluster sizes,
and then a random sample drawn uniformly within the cluster.
(The notation $\mathbb{E}_{( x, y ) \sim C_k}$ denotes averaging over an implicit discrete distribution over the elements in $C_k$.)

One may construct other sampling distributions over the clusters, e.g., of the form $p_k \propto | C_k |^{\alpha}$ for $\alpha \in [ 0, 1 ]$;
this allows for a more diverse mix of clusters in the updates,
at the expense of no longer providing an unbiased estimate of the empirical risk $R( h; S )$.

%
\textbf{\color{Maroon}Remark}.
The current algorithm does not weight based on cluster size. ({\bf\color{red}clarify})
This may potentially introduce some bias.

\

%
\textbf{Connection to existing works}.
Below, we detail some existing works on related problems.

\

%
\emph{Importance weighted SGD}.
Standard SGD iteratively updates a hypothesis based on a minibatch $S_{\rm mb}$ drawn uniformly at random from $S$.
We have $\mathbb{E}[ R( h; S_{\rm mb} ) ] = R( h; S )$, and so the resulting updates are unbiased.
One may however reduce the variance of the updates by instead drawing samples from some non-uniform distribution $p \sim \Delta_{[N]}$;
to preserve unbiasedness, this necessitates scaling the loss by $\frac{1}{p_n}$, i.e.,
$$ \tilde{R}( h; S_{\rm mb} ) = \frac{1}{N_{\rm mb}} \sum_{n \in [N]} \frac{\indicator{(x_n, y_n) \in S_{\rm mb}}}{p_n} \cdot \ell( y_n, h( x_n ) ). $$
Theoretically, to minimise the variance of the resulting gradients, one ought to pick $p_n \propto \| \nabla \ell( y_n, h( x_n ) ) \|_2$,
i.e., one favours samples with higher gradient magnitude~\citep{Zhao:2015}.
This aims to focus attention on ``informative'' samples, and to avoid wasting effort on samples which already possess a low gradient.
In a related approach,~\citet{Zhao:2014} proposed stratified sampling based on clusters, either pre-computed (e.g., via $k$-means) or via an iteration-dependent solution to a certain objective function.
This approach similarly seeks to minimise variance of the SGD updates.

Intuitively, the motivation of margin sampling is to similarly focus attention on informative samples.
Performing round-robin sampling based on clusters has a slightly different motivation, i.e., preventing redundancy in the updates. 
For example, two near-identical samples may each have high gradients, but it may be wasteful to pick both of them when performing an update.

\

%
\emph{Minibatch sampling}.
The above works on importance sampling for SGD endow each input example with a sampling probability.
One may also consider sampling over minibatches themselves.
\citet{Csiba:2018} proposed ``bucket sampling'' based on a partition (``buckets'') of the training samples,
which can lead to provable convergence speedup for SGD.
Empirically, they used random partitions.
Note that unlike~\citet{Zhao:2014}, the sampling is not merely stratified, i.e., within a bucket, one does not simply draw samples uniformly at random.

\citet{Mariet:2020} showed that when sampling with replacement, importance sampling remains optimal even for the minibatch setting.
When sampling without replacement, in general it is NP-hard to find the optimal sampling distribution.
However, motivated by reducing redundancy amongst the samples, the authors attempt to learn a determinantal point process (DPP) based sampling distribution, which inherently allows for diversity amongst the samples.
There is no theoretical analysis of this particular approach, however.


\

%
\emph{Loss proportional sampling}.
\citet{Mineiro:2013} proposed a technique for compressing a dataset in a loss and hypothesis class sensitive manner.
Their formal goal is almost exactly aligned with the one stated above, with an important exception:
they assume that one can use the entire training set $S$.
Indeed, their concern is settings where finding the minimiser $h^*$ is expensive owing to the complexity of optimising with $\mathscr{H}$ (e.g., a deep neural network).
Their basic idea is to consider a suitable subset of hypotheses $\mathscr{H'} \subset \mathscr{H}$, which are more amenable to optimisation (e.g., a linear model).
The resulting minimiser $\tilde{h}$ is then used to inform how to sample points for learning with $\mathscr{H}$.

\

%
\emph{Top-$k$ loss}.
Recall that the above algorithm
retains low-margin samples.
In some settings, these samples cannot consist of low-loss samples.
For example, in a binary setting with convex margin loss $\phi( y \cdot h( x ) )$,
$| h( x ) |$ being small implies a loss value close to $\phi( 0 )$, which may be $\gg \inf_z \phi( z )$.
A related algorithm thus involves discarding low-loss samples, and focussing instead on those samples that the current model is poor at predicting.

This is related to minimising the \emph{average top-$k$} as opposed to the empirical loss,
i.e.,~\citep{Fan:2017}
$$ R( h; S ) = \frac{1}{k} \sum_{i \in [k]} \ell_{[i]}( h; S ), $$
where $\ell_{[i]}( h; S )$ denotes the $i$th largest value of the sample losses $\{ \ell( y_n, h( x_n ) ) \}_{n = 1}^N$.
When $k = 1$, this is the maximum loss over all the training samples.
While potentially susceptible to noise, 
such objectives can be motivated from a \emph{fairness} perspective:
the objective can encourage good performance on rare \emph{subpopulations} within the data~\citep{Shalev-Shwartz:2016}.


\

%
\emph{Coresets}.
The coreset literature is concerned with the problem of finding a subset $S' \subset S$ that can serve as a drop-in replacement for $S$, in the sense of resulting in similar downstream performance~\citep{Bachem:2017}.

\

%
\emph{Negative mining}.
In settings where the number of possible labels is prohibitively large,
computing the loss $\ell( y_n, h( x_n ) )$ on a \emph{single} sample may be prohibitive.
For example, 
under the softmax cross-entropy,
we need to compute $\log\left[1 +  \sum_{y' \neq y_n} e^{h_y( x_n ) - h_{y_n}( x_n )} \right]$, which can be expensive.
This motivates \emph{negative mining} techniques, which draw a sample of ``negative'' labels $\bar{\mathscr{Y}} \subset \mathscr{Y} - \{ y_n \}$,
and compute the loss on this subset.
An example of such a technique is stochastic negative mining~\citep{Reddi:2019},
which first draws a large uniform pool of negatives,
and then retains only the top-$k$ labels with highest loss.

